Preliminary Notes on Termination and Non-Termination Reasoning

In this preliminary note, we will illustrate our ideas on automated mechanisms for termination and non-termination reasoning.

==> fig.scc.tex <==
\begin{figure}[thb]
\begin{small}
\begin{tabular}{ccc}
\begin{array}[t]{l}
\code{\void ~ main ~ () ~ \{}\\
\code{\tab \intr ~ i, ~j, ~n;}\\
\code{\tab i = 0;}\\
\code{\tab \while ~ (i < n) ~\{}\\
\code{\tab \tab j = 0;}\\
\code{\tab \tab \while ~ (j \leq i) ~ \{}\\
\code{\tab \tab \tab j = j + 1; ~\}}\\
\code{\tab \tab i = i + 1; ~ \}}\\
\code{\}}
\end{array}
&
\begin{array}[t]{l}
\code{\void ~ main ~ () ~ \{}\\
\code{\tab \intr ~ i, j, n;}\\
\code{\tab i = 0;}\\
\code{\tab loop_1(i, j, n); ~\}}\\\\

\code{\void ~ loop_1 ~ (\refn ~ \intr ~ i, j, n) ~ \{}\\
\code{\tab \cond ~ (i < n) ~\{}\\
\code{\tab \tab j = 0;}\\
\code{\tab \tab loop_2(i,j);}\\
\code{\tab \tab i = i + 1;}\\
\code{\tab \tab loop_1(i, j, n); ~\}}\\
\code{\tab \ret; ~\}}\\\\

\code{\void ~ loop_2 ~ (\refn ~ \intr ~ i, j) ~ \{}\\
\code{\tab \cond ~ (j \leq i) ~\{}\\
\code{\tab \tab j = j + 1;}\\
\code{\tab \tab loop_2(i, j);~\}}\\
\code{\tab \ret; ~\}}
\end{array}
&
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2cm,
                    semithick]
  %\tikzstyle{every state}=[fill=red,draw=none,text=white]

  \node[initial,state] (A)                    {$main$};
  \node[state]         (B) [below of=A]       {$loop_1$};
  \node[state]         (C) [below of=B]       {$loop_2$};

  \path (A) edge              node {} (B)
        (B) edge [loop left]  node {} (B)
            edge              node {} (C)
        (C) edge [loop left]  node {} (C);
\end{tikzpicture}
\end{tabular}
\end{small}
\end{figure}

